OneFlow: Concurrent Mixed-Modal and Interleaved Generation with Edit Flows

We present OneFlow, the first non-autoregressive multimodal model that enables variable-length and concurrent mixed-modal generation. Unlike autoregressive models that enforce rigid causal ordering between text and image generation, OneFlow combines an insertion-based Edit Flow for discrete text tokens with Flow Matching for image latents. OneFlow enables concurrent text-image synthesis with hierarchical sampling that prioritizes content over grammar. Through controlled experiments across model sizes from 1B to 8B, we demonstrate that OneFlow outperforms autoregressive baselines on both generation and understanding tasks while using up to 50% fewer training FLOPs. OneFlow surpasses both autoregressive and diffusion-based approaches while unlocking new capabilities for concurrent generation, iterative refinement, and natural reasoning-like generation.

==> figures/color_coded_interleaved.tex <==
% Response 3000 Highlighted Tokens
% This file can be included in LaTeX documents using \include{response_3000_highlighted_includable}
% Requires: \usepackage{xcolor}

% The following text represents Response 3000 with tokens highlighted by insertion order
% Blue highlighting for question tokens, yellow gradient for answer tokens based on insertion time

% Colorbar showing yellow gradient for answer tokens (dark = early insertion, light = late insertion)
\colorbox[HTML]{cccc00}{\space{}}\colorbox[HTML]{cece0c}{\space{}}\colorbox[HTML]{d1d118}{\space{}}\colorbox[HTML]{d4d424}{\space{}}\colorbox[HTML]{d6d630}{\space{}}\colorbox[HTML]{d9d93c}{\space{}}\colorbox[HTML]{dcdc48}{\space{}}\colorbox[HTML]{dede54}{\space{}}\colorbox[HTML]{e1e160}{\space{}}\colorbox[HTML]{e4e46c}{\space{}}\colorbox[HTML]{e6e678}{\space{}}\colorbox[HTML]{e9e984}{\space{}}\colorbox[HTML]{ecec90}{\space{}}\colorbox[HTML]{eeee9d}{\space{}}\colorbox[HTML]{f1f1a9}{\space{}}\colorbox[HTML]{f4f4b5}{\space{}}\colorbox[HTML]{f6f6c1}{\space{}}\colorbox[HTML]{f9f9cd}{\space{}}\colorbox[HTML]{fcfcd9}{\space{}}\colorbox[HTML]{ffffe5}{\space{}}


\colorbox[HTML]{87ceeb}{Show}%
\colorbox[HTML]{87ceeb}{\space{}me}%
\colorbox[HTML]{87ceeb}{\space{}a}%
\colorbox[HTML]{87ceeb}{\space{}picture}%
\colorbox[HTML]{87ceeb}{\space{}of}%
\colorbox[HTML]{87ceeb}{\space{}a}%
\colorbox[HTML]{87ceeb}{\space{}cute}%
\colorbox[HTML]{87ceeb}{\space{}dog}%
\colorbox[HTML]{87ceeb}{\space{}to}%
\colorbox[HTML]{87ceeb}{\space{}cheer}%
\colorbox[HTML]{87ceeb}{\space{}me}%
\colorbox[HTML]{87ceeb}{\space{}up}%
\colorbox[HTML]{87ceeb}{.}%
\colorbox[HTML]{f5f5bc}{Here}%
\colorbox[HTML]{cece0c}{'s}%
\colorbox[HTML]{cccc00}{\space{}a}%
\colorbox[HTML]{cccc00}{\space{}picture}%
\colorbox[HTML]{eded98}{\space{}of}%
\colorbox[HTML]{d2d21d}{\space{}a}%
\colorbox[HTML]{cdcd06}{\space{}cute}%
\colorbox[HTML]{e8e87f}{\space{}p}%
\colorbox[HTML]{d5d52c}{ug}%
\colorbox[HTML]{cdcd06}{\space{}in}%
\colorbox[HTML]{d9d93e}{\space{}a}%
\colorbox[HTML]{d2d21b}{\space{}car}%
\colorbox[HTML]{e5e573}{.}%
\colorbox[HTML]{e9e986}{\textless{}\textbar{}image\textbar{}\textgreater{}}%
\colorbox[HTML]{cdcd06}{The}%
\colorbox[HTML]{f6f6bf}{\space{}dog}%
\colorbox[HTML]{cece0c}{'s}%
\colorbox[HTML]{d6d630}{\space{}fur}%
\colorbox[HTML]{d6d630}{\space{}is}%
\colorbox[HTML]{eaea89}{\space{}a}%
\colorbox[HTML]{f9f9cd}{\space{}warm}%
\colorbox[HTML]{d2d21d}{,}%
\colorbox[HTML]{ffffe5}{\space{}golden}%
\colorbox[HTML]{dddd4f}{\space{}color}%
\colorbox[HTML]{cdcd06}{,}%
\colorbox[HTML]{d5d52b}{\space{}with}%
\colorbox[HTML]{d4d425}{\space{}a}%
\colorbox[HTML]{dfdf56}{\space{}cute}%
\colorbox[HTML]{fcfcdb}{,}%
\colorbox[HTML]{d4d425}{\space{}alert}%
\colorbox[HTML]{dada42}{,}%
\colorbox[HTML]{cdcd06}{\space{}and}%
\colorbox[HTML]{d9d93e}{\space{}bright}%
\colorbox[HTML]{d4d425}{\space{}smile}%
\colorbox[HTML]{fefee3}{.}%
\colorbox[HTML]{d4d425}{\space{}I}%
\colorbox[HTML]{d2d21d}{\space{}hope}%
\colorbox[HTML]{d0d014}{\space{}this}%
\colorbox[HTML]{d0d014}{\space{}helps}%
\colorbox[HTML]{cece0c}{\space{}cheer}%
\colorbox[HTML]{f5f5ba}{\space{}you}%
\colorbox[HTML]{fdfdde}{\space{}up}%
\colorbox[HTML]{f7f7c2}{!}%

==> iclr_2026/paper_content.tex <==

\section{Introduction}
Native Multimodal Models — models capable of handling both multimodal understanding and generation within a single backbone — have advanced considerably in visual understanding and generation. These models typically employ a unified transformer architecture with next-token prediction to handle both discrete and continuous generation~\citep{team2024chameleon, janus, janusflow, bagel, transfusion}. Recent work like Transfusion~\citep{transfusion} and Show-O~\citep{showo} demonstrates that leveraging modality-specific training objectives within shared architectures can significantly improve performance, particularly on continuous modalities such as vision.\looseness=-1

However, both autoregressive (\AR) and diffusion-based multimodal approaches face fundamental architectural constraints. Autoregressive models can handle interleaved data but require strict sequential generation — each image must be fully completed before text generation can continue, preventing simultaneous cross-modal refinement. Conversely, diffusion-based multimodal models such as MMaDA~\citep{mmada}, FUDOKI~\citep{fudoki}, and Unidisc~\citep{unidisc} enable simultaneous mixed-modal generation but only for predetermined single text-image pairs where modality assignments must be known a priori and rely on independent time schedules for each modality. Neither paradigm supports the simultaneous generation of variable-length interleaved sequences.\looseness=-1

We present \textbf{\EF}, the first model to achieve simultaneous generation of interleaved data. Unlike autoregressive models that enforce sequential completion of each modality, and unlike diffusion models restricted to fixed length generation, \EF combines an insertion-based discrete text generation using Edit Flows with Flow Matching for image generation. This enables concurrent refinement of both text and images with per-image time schedules, using a novel interleaved time schedule.\looseness=-1

Through controlled experiments across various model sizes and compute regimes, we demonstrate that \EF outperforms both autoregressive (\AR) and diffusion baselines on generation and understanding tasks while requiring 50\% fewer training FLOPs. Moreover, we find that concurrent mixed modal pretraining yields 4\% relative improvement on VQA and 1.5\% on image generation over sequential pretraining. We summarize our contributions below. 


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/figure_1.pdf}
    \caption{OneFlow is a variable-length non-autoregressive model that can concurrently generate interleaved text and variable number of images using insertions as a primitive operation.}
    \label{fig:joint_generation}
\end{figure}

\begin{tcolorbox}[
    colback=blue!5,     % Your specified background color
    colframe=teal!60!black,     % Deep navy frame color
    arc=5pt,                    % Less rounded corners for a modern look
    boxsep=5pt,                 % Inner margin between text and frame
    left=5pt,                   % Reduced left margin within the box
    right=10pt,                 % Right margin within the box
    top=5pt,                    % Top margin within the box
    bottom=5pt,                 % Bottom margin within the box
    boxrule=0.8pt,              % Frame thickness
    drop shadow=gray!50!white,  % Subtle shadow effect for depth
    enhanced jigsaw             % Allows for the shadow effect and better arcs
]
\textbf{Contributions:}
\begin{enumerate}[leftmargin=15pt]
    \item We introduce \EF, a non-autoregressive multimodal model that unifies image and text generation under a simultanous Edit Flow and Flow Matching framework.
    \item \EF enables new capabilities such as concurrent mixed-modal generation, which helps boost performance over uni-modal generation on a wide range of benchmarks.
    \item Through controlled experiences from 1B to 8B, we find that \EF scales better than autoregressive multimodal models, more so with mixed-modal training.
    \item \EF outperforms or is competitive with existing AR and diffusion-based models, on a diverse range of image generation and image understanding benchmarks.
\end{enumerate}
\end{tcolorbox}


% https://docs.google.com/presentation/d/1g6Emlyh7SUfnQpmeh_ipHN7rKoGnULuUGUDCSg8F9Wo/edit?usp=sharing
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{figures/figure_1.pdf}
%     \caption{OneFlow is a variable-length non-autoregressive model that can concurrently generate interleaved text and variable number of images using insertions as a primitive operation.}
%     \label{fig:joint_generation}
% \end{figure}



\section{OneFlow: Mixed-Modal Generation through Flow Matching}

% We aim to generate variable-length, interleaved text–image sequences without autoregression by combining two complementary processes: an Edit Flow model that inserts text tokens or noisy image embeddings during generation, and Flow Matching velocity that denoises continuous image embeddings. 

OneFlow handles multiple modalities through a sequence model, where elements in the sequence can be discrete tokens or continuous embeddings, \eg, of images. Concretely, let $\gT$ denote the space of a single element of the sequence, which can take either a discrete value, up to some fixed vocabulary size $M$, or a continuous value, \ie, $\gT = [M] \cup \R$.
Then our state space is defined as the set of all possible sequences up to some maximum length $N$, \ie, $\gX = \bigcup_{n=0}^N \gT^n$. 

During generation, our model transforms noisy sequences into clean sequences. We do this by combining discrete-valued and continuous-valued generative processes. Specifically, we make use of the Edit Flows~\citep{havasi2025edit} framework which enables variable-length sequence generation through the use of edit operations. It starts with a noisy sequence and iteratively applies edits until it is denoised into a generation. We focus on the \emph{insertion} capabilities of Edit Flows, which is conceptually simple yet extremely powerful, as it allows inserting arbitrary number of tokens---and images---into the generated sequence. When images are inserted, we initialize them with noise and then use Flow Matching~\citep{lipman2024flow} to generate the image. Since the same model predicts both the text edits and the image denoising, OneFlow achieves variable-length, non-autoregressive joint image and text generation. In the following, we state equations with only intuitive justifications and explanations. Full mathematical details and derivations can be found in Appendix~\ref{app:edit_flow_derivation}.

\subsection{Discrete text generation via Edit Flows}

Edit Flows uses a continuous-time Markov chain (CTMC) to iteratively refine variable-length discrete sequences. We start with an empty sequence $X_0 = \emptyset$ at time $t=0$, and transform the sequence through insertion operations. 
Let $\ins(x, i, a)$, $x \in \gX, i \in \{1, \dots, n\}, a \in \gT$, be the sequence resulting from inserting the token value $a$ to the right of position $i$ of the sequence $x$, resulting in
\begin{equation}
    \ins(x, i, a) = (x^1,\dots, x^i, a, x^{i+1}, \dots, x^{n}).
\end{equation}
This forms the primitive operation that we use during generation. 

During training, we take a data sequence $X_1$ and randomly delete tokens with equal probability to obtain $X_t$. This defines the process $X_{[0,1]}$ that we will fit to. The probability of each token being deleted is set by a monotonic scheduler $\kappa_t$ with $\kappa_0=0, \kappa_1=1$.
\begin{equation}\label{eq:schedule}
    \P(x^i \text{ in } X_t) = \kappa_t, \qquad \text{ for each }x^i \in X_1.
\end{equation}
In preliminary experiments, we tested different $\kappa_t$ but found that the linear schedule $\kappa_t = t$ works most consistently across our diverse benchmarks. \textit{Deleted tokens are removed from the sequence}. Noting that on average we retain $\E_t[\kappa_t]$ fraction of the original tokens, with the linear schedule we retain $50\%$ of the data sequence. This can lead to significant FLOPs savings during training, and tuning the scheduler can save even more if desired. 

\textbf{Parameterization.} The parameterization of an Edit Flow model for insertions naturally decomposes into two predictions: (i) how many tokens are missing at the right of position $i$, and (ii) which tokens are missing. 
Thus, at each position $i$ of the sequence, our model outputs two quantities 
\begin{itemize}
    \item $\lambda^i: \mathcal{X} \rightarrow \R^+$ is a scalar that predicts the \emph{number of missing tokens} between $i$ and $i+1$.
    \item $Q^i : \mathcal{X} \rightarrow [M]$ is a normalized distribution that predicts \emph{what tokens are missing}.
\end{itemize}
These two predictions form the CTMC rate and gives the transitions (up to $o(h)$ error),
\begin{equation}\label{eq:sampling_step}
    \P\left(X_{t+h} = \ins(X_t, i, a) \;|\; X_t \right) = h \tfrac{\dot{\kappa}_t}{1 - \kappa_t} \lambda^i(X_t) Q^i (a | X_t).
\end{equation}
The ratio $\tfrac{\dot{\kappa}_t}{1 - \kappa_t}$ dictates the distribution of insertion times according to the schedule $\kappa_t$ imposed during training \eqref{eq:schedule}, where $\dot{\kappa}_t = \tfrac{d\kappa_t}{dt}$.
Note that unlike prior work \citep{havasi2025edit}, we factor out this ratio $\tfrac{\dot{\kappa}_t}{1 - \kappa_t}$ from the rate predictions and use a simplified model that is independent of $t$. Practically, we do not feed time values into the network for predicting insertions. 
While not theoretically justified, we found this $t$-independence assumption to work better in practice, likely because $X_t$ already contains sufficient information for predicting the insertions.

\textbf{Insertion prediction ($\lambda^i$).} The main component that determines whether insertions occur is the prediction head $\lambda^i$, which is trained by regressing onto the number of missing tokens. 
Each position $i$ of the noisy sequence $X_t$ has a corresponding number of missing tokens $k^i$, which is the number of deleted tokens between $X_t^i$ and $X_t^{i+1}$. 
The original Edit Flows loss was constructed through a choice of Bregman divergence \citep{holderrieth2024generator} which results in
\begin{equation}\label{eq:poisson_nll}
    \ell_\text{Poisson}(\lambda^i) = \tsum_i \lambda^i(X_t) - k^i \log \lambda^i(X_t).
\end{equation}
Alternatively, \eqref{eq:poisson_nll} can be interpreted as the negative log-likelihood of a Poisson distribution, so $\lambda^i$ is trained to fit a Poisson distribution to model missing token counts $k^i$. However, the distribution of $k$ has a very high concentration around zero missing count. Furthermore, during sampling, the key prediction is whether the missing token count is zero or nonzero.
As such, we explicitly model the probability of inserting zero tokens.
\begin{equation}
\P(k = 0) = \pi, \quad \text{ and } \quad \P(k) = (1 - \pi) \text{Pois}(k ; \lambda_{\text{nonzero}} \;|\; k > 0) \quad \text{ for $k > 0$}
\end{equation}
\noindent
where $\pi \in (0, 1)$ is the probability of observing zero, and $\lambda_{\text{nonzero}} > 0$ is the rate parameter but restricted to only modeling the distribution of nonzero counts. 
We train $\pi$ by using a binary cross entropy (BCE) loss to detect if the missing count is zero, and we train $\lambda_{\text{nonzero}}$ using the original loss (\eqref{eq:poisson_nll}) on nonzero counts.
For sampling \eqref{eq:sampling_step}, we can use the expectation $\lambda^i(X_t) = (1-\pi^i(X_t)) \lambda^i_{\text{nonzero}}(X_t)$. 
However, we found that a consistently better sampling strategy is to first sample whether there are zero insertions using $\pi$, then simply use the rate $\lambda^i_{\text{nonzero}}(X_t)$ if there are nonzero insertions.

\textbf{Bag-of-tokens prediction ($Q^i$).} To determine what token to insert at each position, we make use of the output head $Q$ which is a softmax over the discrete vocabulary $[M]$. We use the same Edit Flows loss, which is a sum of cross-entropy loss. Let $\mathcal{A}_i$ denote the set of deleted tokens between $X_t^i$ and $X_t^{i+1}$, then for each position $i$, the loss is
\begin{equation}\label{eq:token_loss}
    \ell_{\text{tokens}}(Q^i) = - \tsum_{a \in \mathcal{A}_i} \log Q^i(a | X_t).
\end{equation}

\textbf{Combined loss.} At each training iteration, we randomly delete tokens from the data sequence, and learn to predict the set of missing tokens at each position, resulting in the total insertion loss:
\begin{equation}\label{eq:insertion_loss}
    \mathcal{L}_{\text{text}} = \E_{t, X_t | X_1} \left[ \frac{1}{n} \sum_{i=1}^{n} \ell_{\text{tokens}}(Q^i) + \ell_\text{Poisson}(\lambda^i_\text{nonzero}) \1_{[k_i > 0]} + \ell_\text{BCE}(\pi^i) \right]
\end{equation}
where $n$ is the length of the noisy sequence $X_t$. Note that this differs from the original training objective in Edit Flows \citep{havasi2025edit} which additionally weights the loss by the factor $\tfrac{\dot{\kappa}_t}{1 - \kappa_t}$, not affecting the optimal solution. We found that not using this factor produces better results.

\subsection{Continuous image generation via Flow Matching}

Following standard practice, we generate images starting from a Gaussian noise of fixed dimension $N_{\text{img}}$, applying a deterministic generation procedure that follows an ordinary differential equation. Let $Y_t \in \R^{N_{\text{img}}}$ denote the noisy image, then the generative process is
\begin{equation}
    \tfrac{d}{dt} Y_t = v(Y_t, t), \qquad Y_0 \sim \mathcal{N}(0, I),
\end{equation}
where $v: \R^{N_{\text{img}}}\times\R \rightarrow \R^{N_{\text{img}}}$ is a velocity field that determines the direction to transform $Y_t$ into a clean sample by $t=1$.
During training, we sample a noise $Y_0$ and obtain $Y_t$ with a linear schedule $Y_t = tY_1 + (1-t)Y_0$. The Flow Matching loss can then be written as
\begin{equation}\label{eq:flow_matching}
    \mathcal{L}_\text{image} = \E_{t, Y_0, Y_1} \left\lVert v(Y_t, t) - (Y_1 - Y_0) \right\rVert^2.
\end{equation}
In OneFlow, we use a pretrained autoencoder to map images into latent space. We then design the velocity network $v(\cdot)$ to use a shared Transformer backbone as text but with additional U-Nets to downsample and upsample between the backbone and autoencoder embedding spaces, making use of the same architectural design as Transfusion~\citep{transfusion}. See illustration in Figure \ref{fig:architecture}.

\subsection{Concurrent Mixed-modal Generation}\label{sec:mixed_modal_schedules}

To generate multiple modalities, we simply concatenate them into a single sequence. We now present two multimodal time schedules, an independent schedule that can be used when the number of images is known, and an interleaved schedule that needs to be used when the number of images is arbitrary. OneFlow is designed to work with variable-length text and variable number of images.

\textbf{Independent mixed-modal generation.}
We can consider the simple case with a fixed number of images---typically one. In such case, we can generate both the text and image simultaneously by using two time values $t_\text{text}$ and $t_\text{img}$, where $t_\text{text}$ determines the state of the insertion generation process and $t_\text{img}$ determines the image generation process. 
Following prior work, we simply set independent time schedules, one for the text and one for each image. This allows the modalities to be concurrently generated and be dependent on each other during the generation process. However, this na\"ive process does not allow us to insert images.

\textbf{Interleaved mixed-modal generation.}
A much more complicated setting arises when the number of images is variable and images are being inserted as part of the generation process. Similar to the text-only setting, we start generating from the empty sequence.
We then model image insertion as a special token value \image, which is added to the token prediction output $Q$.
During generation, when the model predicts an image insertion, we insert noise embeddings of dimension $N_{\text{img}}$ into the sequence to represent an inserted image initialized at $t_\text{img} = 0$. 
\begin{equation}
    \ins(x, i, \image) = \big(x^1,\dots, x^i, x^1_\text{img}, \dots, x_\text{img}^{N_\text{img}}, x^{i+1}, \dots, x^{n}\big), \qquad x^i_\text{img} \sim \mathcal{N}(0, I).
\end{equation}
Subsequent steps during generation would then simultaneously generate the image embeddings while also performing more insertions into the sequence. However, since the image is generated at a later time, this implies there is a delay between the image time and the text time, \ie $t_\text{img} \leq t_\text{text}$, which needs to be taken into account during training.

During training, we need to ensure that the text and image noise levels are consistent with with the ones seen during generation. 
Based on the schedule in \eqref{eq:schedule}, the time at which an insertion happens is a random variable that has $\kappa$ as its cumulative density function, so the time difference between the inserted image time $t_\text{img}$ and the initial text time $t_\text{text}$ is given by
\begin{equation}\label{eq:interleaved_time_schedule}
    t_\text{img} = t_\text{text} - \kappa^{-1}(u), \qquad \text{ where } u \sim \text{Unif(0, 1)}.
\end{equation}
We call this the \emph{interleaved time schedule}, which imposes a distributional dependency between the time values $t_\text{img}$ for each image and the text time $t_\text{text}$. 
In order for the model to learn to fully generate all images, during training we sample from an extended time interval, $\tau_{\text{text}}$ from $[0, 2]$, since the \image token can be inserted at $\tau_{\text{text}}=1.0$ at the latest, and fully denoised by $\tau_{\text{text}}=2.0$. The probability for each token being in $X_t$ is then determined by $\kappa(\min\{1, \tau_{\text{text}}\})$ in place of \eqref{eq:schedule}.
We also sample for each image an extended time value $\tau_{\text{img}} = \tau_\text{text} - \kappa^{-1}(u)$. 
Finally, we determine if an image is deleted from the sequence by checking $\tau_{\text{img}} < 0$, and if so, the insertion loss (\eqref{eq:insertion_loss}) will include the \image{} token which the model would learn to insert. Otherwise if $\tau_{\text{img}} \geq 0$, the image is in the sequence and we set $t_\text{img} = \min\{1, \tau_{\text{img}}\}$; using the Flow Matching loss \eqref{eq:flow_matching} to train the velocity. A detailed derivation and more in-depth explanation can be found in Appendix \ref{app:interleaved_schedule}.

\input{tables/image_gen_controlled}
\section{Experiments}
We present our experimental results through five research questions: \S \ref{controlled} How does \EF perform compared to \AR, and does it scale similarly? \S \ref{sec:mixed_modal} How does mixed modal pretraining compare to sequential pretraining? \S \ref{sec:vqa_sampling} Why does \EF outperform \AR in text generation? \S \ref{sec:comparison} How does \EF compare against other unified multimodal models? Finally, \S \ref{sec:interleaved} What new capabilities does \EF unlock?

\textbf{Training stages.}
Our training consists of two main stages: multimodal pretraining and instruction finetuning. During the pretraining stage, we use a mixture of image understanding and image generation data to learn representations for both image and text. We trained with a sequence length of 512 and a global batch size of 4096. We can set the mixed generation probability (the likelihood of concurrently generating clean text and images from a noisy input) to be either 0 or 0.2.

For finetuning, we use a mixture of VQA, text, and interleaved data to give the model the ability to respond to visual question answering problems. We also fine-tune on image generation data at a higher resolution of 512$\times$512 to improve the model’s image generation capabilities. We study the model's behavior at the 1B scale for our ablations and controlled experiments, and the scaling trend up to 8B is detailed in Section~\ref{controlled}.

\textbf{Datasets.}
For multimodal pretraining, we use image-text pairs from a filtered version of the Conceptual Captions dataset (CC12M \citep{sharma2018conceptual}), the YFCC dataset \citep{thomee2016yfcc100m}, and licensed data, for a total of 400M examples. During instruction finetuning, we use a filtered image portion of the PerceptionLM dataset \citep{cho2025perceptionlm}, interleaving data from Chameleon \citep{team2024chameleon}, and Cambrian-7M~\citep{tong2024cambrian} dataset. 

\textbf{Baselines.} To evaluate our model's performance against existing methods, we compare against two baselines: (1) an autoregressive (\AR) + Flow Matching (FM) multimodal model based on Transfusion~\citep{transfusion}, where text tokens are generated autoregressively and image tokens via FM, and (2) a masked diffusion model based on LLaDA~\citep{nie2025large}. For the masked diffusion baseline, we tested two sampling variants: low-confidence and random remasking, with random remasking performing better across all experiments. Unlike Transfusion, we follow Janus-Flow~\citep{janusflow} and adopt a dual-encoder setup. For image encoders, we use a pretrained SigLIP2 ViT-SO400M-16@512~\citep{siglip2} for understanding and an SD3 VAE~\citep{sd3} for generation. Following Transfusion, we use U-Net adapters.

\input{tables/vqa_controlled}

\textbf{Evaluation setup.}
Following Cambrian~\citep{tong2024cambrian} and PLM~\citep{cho2025perceptionlm}, we group VQA tasks into five groups: General, Knowledge, OCR \& Chart, Hard Perception, and Hallucination. We evaluate image generation quality using FID~\citep{fid} on COCO-2014~\citep{coco2014} validation set. To assess prompt alignment, we report CLIPScore~\citep{clipscore} and DPG-Bench~\citep{dpgbench}. Additionally, we include WISE~\citep{wise} cultural to better understand knowledge-based generation.




\subsection{\EF Scales Better Than \AR}
\label{controlled}
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/scaling.pdf}
    \caption{\textbf{Performance of \EF vs. \AR baseline models at different model scales, data and compute.} For text-to-image generation, we report DPG-Bench and FID. For image-to-text caption quality, we report CIDEr and ROUGE.  In every benchmark, \EF consistently exhibits better scaling laws than \AR.}
    \label{fig:scaling_pretraining}
    \vspace{-15pt}
\end{figure*}

In this experiment, we study the performance of \EF and \AR in controlled settings at various model sizes and token counts. To ensure \EF has no advantage in data-constrained settings, we trained both models on 2B image-text pairs over 500k iterations using a batch size of 4096. Both models were initialized from Llama 3.2 1B~\citep{llama3modelcard}. For AR, the number of tokens predicted during training equals the sequence length, whereas for OneFlow, the number of predicted tokens corresponds to the number of deleted tokens, which on average is 50\% of the data sequence.

We find that \EF scales better than \AR on every benchmark. This scaling advantage is especially pronounced on DPG Bench, where \EF scales significantly better than \AR. Conversely, for image captioning, \EF shows a notable performance gap relative to \AR. Figure \ref{fig:scaling_pretraining} visualizes the scaling trend, and the final metrics after training are shown in Table \ref{tab:pretraining_metrics}, along with a comparison against other state-of-the-art models. We provide qualitative examples of where \EF outperforms \AR in Appendix \ref{appendix:qualitative_img_gen}.


\subsection{Mixed Modal Pre-training Enables Better Generation and Understanding}
\label{sec:mixed_modal}

\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{figures/mixed_vs_clean.pdf}
    \caption{\textbf{Mixed modal vs Sequential pretraining.} Mixed modal pretraining vs sequential pretraining. Mixed pretraining achieves 4\% relative improvement on VQA tasks and slight improvements on image generation as well.}
    \label{fig:mixed_vs_clean}
    \vspace{-15pt}  % Reduce bottom spacing
\end{figure}

\begin{wrapfigure}[7]{r}{0.45\textwidth}
    \vspace{-25pt}
    \centering
    \includegraphics[width=0.45\textwidth]{figures/mixed_gen_illustration.pdf}
    \caption{Mixed modal concurrent training.}
    \vspace{-15pt}  % Reduce bottom spacing
    \label{fig:mixed_gen}
\end{wrapfigure}
In this section, we study the impact of mixed modal pretraining. We investigate whether concurrent mixed modal pretraining and sequential pretraining affect downstream understanding tasks. We train two 1B variants: one using sequential pretraining (T2I or I2T), and another with the same data but where 20\% of examples use concurrent generation. Figure~\ref{fig:mixed_vs_clean} indicates that when starting from a concurrent model, downstream image understanding improves by 5\% relatively. These results demonstrate the impact of  concurrent mixed modal pre-training dense prompt alignment.
We also finetune the pretrained model from Section~\ref{controlled} on a mixture of interleaving data, filtered PLM data, and text data to evaluate downstream performance.


\subsection{Hierarchical Generation Enables Reasoning}
\label{sec:vqa_sampling}

\begin{wrapfigure}[17]{r}{0.5\linewidth}
    \centering
    \vspace{-15pt}
    \includegraphics[width=\linewidth]{figures/vqa_viz.pdf}
    \caption{\textbf{\EF response to visual question.} Implicit visual reasoning in hierarchical generation. \EF naturally develops reasoning chains without CoT prompting.}
    \label{fig:vqa_viz}
    \vspace{-15pt}
\end{wrapfigure}

In Figure~\ref{fig:vqa_viz}, we present \EF's sampling process when prompted with a visual question. In response to prompts such as \textit{" \{question\} Explain why."}, \EF generates a reasoning chain before arriving at the final answer, without any Chain-of-Thought (CoT)~\citep{cot} prompting or RL post-training. For example, when asked \textit{"Is there a snowboard in the image? Explain why."}, the model first implicitly performs visual search by examining the image and searching through likely locations for the snowboard. Similarly, for the math puzzle in (Figure~\ref{fig:vqa_viz} bottom), the model first identifies objects in the image that match the prompt description—the green sphere and the large shiny cylinder—before arriving at the final answer.

Our results align with findings in Physics of LLMs~\citep{physics_of_llm} and MetaMorph~\citep{metamorph}, where the authors suggest that LLMs precompute reasoning graphs before generating tokens. However, our findings demonstrate that the model can perform the same reasoning chain without autoregressive decoding. This suggests that reasoning capabilities can emerge in non-autoregressive architectures and transfer effectively to \EF. We show more example VQA generations compared to the AR baseline in Figure \ref{fig:vqa_qualitative_comparison}.


\subsection{Comparison with State-of-The-Art Unified Models}
\label{sec:comparison}

We compare \EF with other autoregressive and diffusion multimodal models and summarize the results in Table~\ref{tab:performance_comparison}. Since these models were trained on different datasets and with different base LLMs, a controlled comparison is difficult. This is why we trained our own autoregressive multimodal model for a fair, apples-to-apples comparison in the previous section.

\EF achieves competitive performance on understanding and generation benchmarks, matching the performance of other state-of-the-art models. For instance, models like MMaDA underwent extensive post-training and reasoning training, while \EF did not. Similarly, FUDOKI was initialized from a pretrained multimodal model, whereas ours was trained from scratch.

\subsection{New Capabilities Introduced by OneFlow}

\paragraph{Classifier-free guidance improves text detailedness.}
\input{figures/cfg_captioning}
% \input{tables/cfg_gpt4}
The use of continuous-time Markov chains allows us to apply classifier-free guidance (CFG) to our model's insertion rates. 
Specifically, given an unconditional prediction $\lambda(X_t)Q(X_t)$ and a conditional prediction $\lambda(X_t | c)Q(X_t | c)$, where $c$ is the prompt and $w$ is the guidance weight, the modified insertion rate is constructed as:
\begin{equation}
    \lambda^\text{cfg}(X_t | c) = \lambda(X_t | c)^w \lambda(X_t)^{1-w} \quad \text{ and } \quad Q^\text{cfg}(X_t | c) \propto Q(X_t | c)^w Q(X_t)^{1-w}.
\end{equation}

As shown in Figures~\ref{fig:image_caption_generation} and \ref{fig:image_caption_generation_more}, higher CFG values consistently increase the length and detail of generated text. We quantitatively evaluated caption quality and hallucination using CapArena~\citep{caparena} by prompting GPT4-o. Our findings show that increasing CFG leads to more detailed captions, with \EF matching \AR's level of detail at a guidance scale of 1. However, this increased detail comes at the expense of hallucinations at very high CFG values.

\paragraph{Simultaneous generation of interleaved text and images.}
\label{sec:interleaved}
When autoregressive multi-modal models insert an image, they append it at the end of the current generation, fully denoise it, then continue the generation process. However, OneFlow is able to simultaneously denoise images and the text. When the model deems it necessary, it is able to insert an new image in the existing text and denoise it along with the text, as proposed in Section \ref{sec:mixed_modal_schedules}.
%
% To achieve this, we treat the image token as any other insertable token. When the model inserts an image token, we include a fully noised image in $X_t$. In each step, the model currently predicts both the text edits and all the image velocities in $X_t$. Note that the text is fully denoised by $t=1$, but the model needs to continue denoising the already existing images until they finish denoising (which is at $t=2$ the latest, in case an image is inserted at $t=1$). 
% Figure \ref{fig:interleaved_generation} demonstrates the interleaved generation process discussed in Section \ref{sec:mixed_modal_schedules}.

To train this model, we took OneFlow 1B Mixed and finetuned it on the interleaved subset of the Chameleon dataset \citep{team2024chameleon} for $20000$ steps. This subset contains $17000$ examples that interleave both text and image data. 
% There are no established benchmarks that directly measure the cohesiveness of join image and text generation, so we rely on qualitative examples to demonstrate this capability. 
Figure \ref{fig:color_coded_example} shows the generation order of the tokens where two images were generated as part of the answer, with more detailed examples in Appendix \ref{sec:further_interleaved} and animated versions in the supplementary material.

\input{tables/color_example} 


\section{Related Work}
\vspace{-0.5em}

\textbf{Native Multimodal Models.} 
Current approaches for unified multimodal models fall into three main paradigms: fully autoregressive \citep{team2024chameleon,emu3,janus}, hybrid \citep{transfusion,bagel,showo,janusflow}, and fully diffusion-based \citep{mmada,unidisc,ddit,fudoki}. While these models are limited by a fixed generation order or fixed-length output, our approach fundamentally differs by being able to simultaneously generate interleaved content and a variable number of images. For a more comprehensive analysis, see Appendix~\ref{sec:appendix_related_works}.

\textbf{Discrete Diffusion and Discrete Flow Matching.} 
Iterative refinement models, including diffusion \citep{sohl2015deep,ho2020denoising} and flow models \citep{liu2022flow,albergo2023stochastic,lipman2024flow}, have been adapted for discrete token spaces. Discrete diffusion models typically learn to reverse a corruption process \citep{austin2021structured,lou2024discrete}, while discrete flow models transport between two distributions with an interpolating scheme \citep{campbell2024generative,gat2024discrete}. Although these frameworks offer a large design space \citep{shaul2024flow, fudoki}, recent works have predominantly focused on a simplified mask construction \citep{sahoo2024simple,shi2024simplified,ou2024your,zheng2024masked}. This masking framework, however, cannot be easily applied to variable-length and especially simultaneous interleaved generation. 
%In contrast, our approach is designed to work easily with any modality, including variable-length representations such as text and a variable number of images.

\textbf{Edit-based Non-autoregressive Language Models.} 
Early non-autoregressive models for variable-length generation \citep{gu2019insertion,gu2019levenshtein,stern2019insertion,reid2022diffuser} often relied on multiple models and evaluations to handle edit operations. While later work like Edit Flows \citep{havasi2025edit} improved on this by using a continuous-time framework and using only a single evaluation per step. \citet{campbell2024trans} also proposed modeling insertions with a diffusion model for denoising, but did not consider sequential data.
In contrast, our approach considers sequential mixed-modal data, allows for parallel token insertions, and uses a unified backbone architecture.

\section{Conclusion and Limitations}
\vspace{-0.5em}

We introduced \EF, a novel non-autoregressive multimodal model that overcomes the fixed-length generation limitations of diffusion models and has better scaling than autoregressive multimodal models. 
We introduced mixed-modal generation approaches, which through extensive controlled experiments,  improve on benchmarks for both image understanding and image generation. 
We also propose a novel approach to interleaved generation that simultaneously denoises images and inserts text tokens, with promising qualitative results. Interleaved generation is still in its infancy and we expect to see more incoming research efforts in constructing large-scale data sets~\citep{mint,obelics,mmc4} and designing comprehensive benchmarks.

A limitation of requiring bidirectional attention is the lack of key-value caching, which increases inference cost. Although we do find that OneFlow can obtain good captioning performance with very few model evaluations---outperforming AR with only 6 sampling steps (Figure \ref{fig:sampling_steps})---it is still slower and more memory-intensive compared to key-value cached autoregressive sampling. Reducing inference costs, with semi-autoregressive models \citep{arriola2025block,gat2025set} or more sophisticated methods, would be an exciting research direction.

% we enable the simultaneous interleaving of images and text. Through extensive controlled experiments, we find that \EF outperforms both masked diffusion and \EF baselines while unlocking a new paradigm for simultaneous interleaved generation.

% While most diffusion multimodal models claim higher sampling efficiency than \AR models, these claims often do not account for the significant speedup provided by key-value caching in \AR sampling. 
% In Appendix \ref{sec:sampling step}, Figure \ref{fig:sampling_steps} shows that few steps is needed to generate decent text; however, a key challenge is that our model currently lacks key-value caching due to its bidirectional attention, which prevents it from sampling efficiently. Improving the sampling efficiency of insertion-based models remains a challenging research question.

% While we have shown the capabity of simultaneous interleaved generation, there are no established benchmarks that directly measure the cohesiveness of joint image and text generation, so we rely on qualitative examples to demonstrate this capability. Further investigation into benchmarks and use cases for interleaved generation can is an exciting research direction to explore.






==> tables/cfg_gpt4.tex <==
\begin{wraptable}{r}{0.4\textwidth}
\vspace{-15pt}
\renewcommand{\arraystretch}{1.1}
\centering
\scriptsize
\begin{tabular}{@{}cccccc@{}}
\toprule
\textbf{CFG Scale} & \textbf{0.0} & \textbf{1.0} & \textbf{1.4} & \textbf{2.0} & \textbf{AR} \\
\midrule
\textbf{GPT Score} & 5.36 & 5.61 & 5.53 & 5.44 & 5.60 \\
\bottomrule

\end{tabular}
\caption{CFG effect on GPT-4 scores.}
\label{tab:cfg_effect}
\vspace{-15pt}  % Reduce bottom spacing
\end{wraptable}

==> tables/geneval.tex <==

\begin{table}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lccccccc@{}}
\toprule
\textbf{Model} & \textbf{Single Object} & \textbf{Two Object} & \textbf{Color Attr.} & \textbf{Position} & \textbf{Colors} & \textbf{Counting} & \textbf{Overall} \\
\midrule
Mixed-modal AR & 90.62\% & 40.40\% & 20.70\% &  9.48\% & 70.63\% & 33.75\% & 0.443 \\
OneFlow & 95.00\% & 57.07\% & 30.92\% & 25.69\% & 75.13\% & 32.81\% & 0.528 \\
OneFlow (mixed gen.) & 82.19\% & 38.13\% & 25.94\% & 10.47\% & 66.93\% & 28.44\% & 0.420 \\
\bottomrule
\end{tabular}
}
\caption{Performance of three models across six evaluation tasks. Overall is the average score across tasks.}
\label{tab:geneval_models}
\end{table}


==> tables/gpt4_prompt.tex <==
\begin{figure*}[!p]
    \centering
    \fbox{
    \begin{minipage}{0.9\textwidth}
        \colorbox{black}{\textcolor{white}{\textbf{Template prompt of VLM-as-a-Judge}}}
        
        \vspace{0.3cm}
        
        Please act as an impartial judge and evaluate the quality of the following caption provided by an AI assistant for a given image.
        
        Begin your evaluation by providing a short explanation. Be as objective as possible. After providing your explanation, please rate the response on a scale of 1 to 10 by strictly following this format: ``[[rating]]'', for example: ``Rating: [[5]]''.
        
        \vspace{0.2cm}
        
        Below are some guidelines for your reference:
        
        \begin{enumerate}
            \item \textbf{Precision}: The caption should accurately correspond to the content of the image, providing precise information about it. Common examples of imprecision include errors in color, quantity, spatial relationships, or the posture of people.
            
            \item \textbf{Informativeness}: Salient information in the image should be reflected in the caption. Since it is impossible to include every detail, you will need to subjectively judge which aspects of the image are important. For instance, describing an otter as ``a small animal'' is precise, but it is less informative than specifying ``an otter''.
            
            \item \textbf{Hallucination}: Captions that include descriptions of objects or elements that are clearly absent from the image should be significantly penalized.
            
            \item \textbf{Attention to detail}: Annotators should pay close attention to the details in the image to distinguish the quality of the descriptions.
            
            \item \textbf{Assistive description}: Imagine a visually impaired person asking you to describe the image for them. How would you convey the image to them?
            
            \item \textbf{Reverse thinking}: What image does the caption lead us to imagine? Does the caption effectively lead you to imagine the intended image?
        \end{enumerate}
        
        \vspace{0.2cm}
        Image: $<$image$>$
        Reference Caption: $<$reference caption$>$
        Caption: $<$caption text$>$
    \end{minipage}
    }
    \caption{Template prompt of VLM-as-a-Judge, taken from \citet{caparena}}
    \label{fig:vlm_judge_template}
\end{figure*}

==> tables/image_gen.tex <==
\begin{table}
\renewcommand{\arraystretch}{1.05}
\centering
\scriptsize
\begin{tabular}{@{}l c cc cccc ccc c@{}}
\toprule
& & & & \multicolumn{4}{c}{\cellcolor{colGen}\textbf{Image Generation}} & \multicolumn{3}{c}{\cellcolor{colHalluc}\textbf{Captioning}} \\
\cmidrule(lr){5-8} \cmidrule(lr){9-11} 
\textbf{Model} & \textbf{Size} & \rotatebox{45}{\textbf{Text}} & \rotatebox{45}{\textbf{Image}} & 
\cellcolor{colGen}\textbf{FID$\downarrow$} & 
\cellcolor{colGen}\textbf{CLIP$\uparrow$} & 
\cellcolor{colGen}\textbf{DPG$\uparrow$} & 
\cellcolor{colGen}\textbf{Wise (c.) $\uparrow$} & 
\cellcolor{colHalluc}\textbf{CDr$\uparrow$} & 
\cellcolor{colHalluc}\textbf{RGE$\uparrow$} &
\cellcolor{colHalluc}\textbf{BLEU4$\uparrow$} \\
\midrule
\multicolumn{11}{l}{\textit{Unified MLM}} \\
Bagel~\citep{bagel} & 7B & AR & FM & 27.7$^\dagger$ & 26.2$^\dagger$ &  \cellhi 84.7$^\dagger$ & 0.44 $^*$& -- & -- & -- \\
MetaMorph~\citep{metamorph}& 7B & AR & AR & 11.8 & 26.6 & -- & -- & -- & -- & -- \\
LMFusion~\citep{lmfusion}  & 7B & AR & Diff & 14.0 & 24.4 & -- & -- & 38.4 & -- & -- \\
Transfusion~\citep{transfusion} & 7B & AR & Diff & 16.0 & 26.5 & 77.8 & -- & 33.7 & -- & -- \\
Janus-Flow~\citep{janusflow} & 1.5B & AR & FM & 12.4$^\dagger$  & 26.1 $^\dagger$ & 80.1 $^\dagger$  & 0.13$^*$ & -- & -- & -- \\
\midrule
\multicolumn{11}{l}{\textit{Multimodal Diffusion}} \\
UniDisc~\citep{unidisc} & 1.4B & Mask & Mask & 23.9 & -- & -- & -- & -- & -- & -- \\
D-DiT~\citep{ddit}  & 2B & Mask & Diff & -- & -- & -- & -- & 56.2 & -- & -- \\
Muddit~\citep{muddit} & 1B & Mask & Mask & -- & -- & -- & -- & 59.7 & -- & --\\
FUDOKI~\citep{fudoki} & 1.5B & DFM & DFM & -- & -- & 83.6 & -- & -- & -- & -- \\
MMaDA~\citep{mmada}  & 8B & Mask & Mask & 33.2$^\dagger$ & 25.1$^\dagger$ & 74.2 $^\dagger$& 0.67$^*$ & -- & -- & -- \\
\midrule
AR-FM Ablation & 1B & AR & FM & 12.2 & 26.5 & 73.4 & 0.61 & 123.9 & 57.2 & 0.39 \\
\textbf{OneFlow 1B} & 1B & EF & FM & 12.1 & 26.6 & 79.1 & 0.62 & 138.1 & 60.8 & 0.41 \\
\textbf{OneFlow Mixed 1B} & 1B & EF & FM & 9.7 & 26.6 & 80.3 & 0.63 & 139.8 & 60.9 & 0.42 \\
\midrule
\textbf{OneFlow 8B} & 8B & EF & FM & 10.7 & \cellhi 26.7 & 79.3 & 0.65 & 141.1 & 61.1 & 0.42 \\
\textbf{OneFlow Mixed 8B} & 8B & EF & FM & \cellhi 9.5 & 26.6 & 80.4 & \cellhi 0.68 & \cellhi 142.1 & \cellhi 61.1 & \cellhi 0.43 \\
\bottomrule
\end{tabular}
\caption{Image generation and captioning benchmarks after multimodal pretraining. Since models are trained on different datasets, and based LMs, an apples-to-apples comparison is difficult. Thus we trained our own \AR-FM model as controlled experiment against our \EF model. }
\label{tab:pretraining_metrics}
\end{table}

==> tables/vqa.tex <==
\begin{table}
\centering
\renewcommand{\arraystretch}{1.1}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{
    l c
    c c c c
    c c
    c c c
    c
    c
}
\toprule
& & 
\multicolumn{4}{c}{\cellcolor{colGen}\textbf{General}} &
\multicolumn{2}{c}{\cellcolor{colKnow}\textbf{Knowledge}} &
\multicolumn{3}{c}{\cellcolor{colOCR}\textbf{OCR \& Chart}} &
\cellcolor{colVision}\textbf{Vision} &
\cellcolor{colHalluc}\textbf{Halluc.} \\
\cmidrule(lr){3-6} \cmidrule(lr){7-8} \cmidrule(lr){9-11} \cmidrule(lr){12-12} \cmidrule(lr){13-13}
\textbf{Model} & \rotatebox{45}{\textbf{Params}} 
& \cellcolor{colGen}\rotatebox{90}{\textbf{MMB}} 
& \cellcolor{colGen}\rotatebox{90}{\textbf{VQAv2}} 
& \cellcolor{colGen}\rotatebox{90}{\textbf{GQA}} 
& \cellcolor{colGen}\rotatebox{90}{\textbf{MME}} 
& \cellcolor{colKnow}\rotatebox{90}{\textbf{MMMU}} 
& \cellcolor{colKnow}\rotatebox{90}{\textbf{AI2D}} 
& \cellcolor{colOCR}\rotatebox{90}{\textbf{DocVQA}} 
& \cellcolor{colOCR}\rotatebox{90}{\textbf{ChartQA}} 
& \cellcolor{colOCR}\rotatebox{90}{\textbf{TextVQA}} 
& \cellcolor{colVision}\rotatebox{90}{\textbf{RealWorldQA}} 
& \cellcolor{colHalluc}\rotatebox{90}{\textbf{POPE}} 
\\
\midrule
\multicolumn{13}{l}{\textit{\color{gray}Und. Only}} \\
\color{gray} PLM 1-tile $^\dagger$ & \color{gray}1B & \color{gray}68.5 & \color{gray}70.1 & \color{gray}57.6 & \color{gray}1410.7 & \color{gray}31.2 & \color{gray}83.3 & \color{gray}51.2 & \color{gray}58.6 & \color{gray}81.2 & \color{gray}62.5 & \color{gray}85.7 \\
\midrule
\multicolumn{13}{l}{\; \textit{Multimodal LM}} \\
Janus-Flow $^*$ & 1.5B & 74.9 & 79.8 & 60.3 & 1333.1 & 29.3 & -- & 64.6 & 55.5 & -- & -- & 88.0 \\
Janus-Pro $^\dagger$ & 1.5B & 73.4 & 67.9 & 59.3 & 1443.0 & 33.4 & 62.8 & 21.2 & 35.8 & 53.9 & 53.5 & 84.8 \\
Janus-Pro $^\dagger$ & 7B & 76.9 & 74.1 & 62.0 & 1531.0 & 38.2 & 68.1 & 24.3 & -- & 57.2 & 56.4 & 85.2 \\
Show-O $^*$ & 1.3B & -- & -- & 61.0 & 1232.9 & 27.4 & -- & -- & -- & -- & -- & 84.5 \\
MetaMorph $^*$ & 7B & 75.2 & -- & -- & -- & 41.8 & -- & -- & 37.1 & 60.5 & 58.3 & -- \\
\midrule
\multicolumn{13}{l}{\; \textit{Mask Diffusion}} \\
Muddit $^*$ & 1B & -- & 67.7 & 57.1 & 1104.6 & -- & -- & -- & -- & -- & -- & -- \\
D-Dit $^*$ & 2B & -- & 60.1 & 59.2 & 1124.7 & -- & -- & -- & -- & -- & -- & 84.0 \\
MMADA $^*$ & 8B & 68.5 & 76.7 & 61.3 & -- & 30.2 & -- & -- & -- & -- & -- & 86.1 \\
\multicolumn{13}{l}{\; \textit{Discrete Flow}} \\
FUDOKI $^*$ & 1.5B & 73.9 & -- & 57.6 & 1485.4 & 34.3 & -- & -- & -- & -- & -- & 86.1 \\
\midrule
AR-FM Ablation & 1B & 54.6 & 64.4 & 53.4 & 1338.7 & 25.7 & 41.9 & 20.9 & 35.1 & 47.6 & 37.6 & 82.8 \\
\rowcolor{blue!5}  \textbf{\EF} & 1B & 71.9 & 68.8 & 57.7 & 1540.6 & 31.1 & 58.5 & 23.2 & 33.8 & 49.5 & 53.3 & 85.7 \\
\rowcolor{blue!5}  \textbf{\EF} & 8B & 72.5 & 73.7 & 61.9 & 1542.5 & 33.1 & 63.4 & 37.1 & 42.1 & 58.6 & 54.0 & 86.3 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{\textbf{Comparison of \EF with other unified models.} \EF offers competitive performance compared to
other leading unified models. Models in gray are understanding-only. $^*$ We use numbers reported in original papers. $^{\dag}$ We obtain results using official open-sourced model weights. \john{cite the models}}

\label{tab:performance_comparison}
\end{table}
